LiDARDraft: Generating LiDAR Point Cloud from Versatile Inputs

Generating realistic and diverse LiDAR point clouds is crucial for autonomous driving simulation. Although previous methods achieve LiDAR point cloud generation from user inputs, they struggle to attain high-quality results while enabling versatile controllability, due to the imbalance between the complex distribution of LiDAR point clouds and the simple control signals. To address the limitation, we propose LiDARDraft, which utilizes the 3D layout to build a bridge between versatile conditional signals and LiDAR point clouds. The 3D layout can be trivially generated from various user inputs such as textual descriptions and images. Specifically, we represent text, images, and point clouds as unified 3D layouts, which are further transformed into semantic and depth control signals. Then, we employ a rangemap-based ControlNet to guide LiDAR point cloud generation. This pixel-level alignment approach demonstrates excellent performance in controllable LiDAR point clouds generation, enabling "simulation from scratch", allowing self-driving environments to be created from arbitrary textual descriptions, images and sketches.

==> sec/6_Limitation.tex <==
\section{Limitation}
We have demonstrated the powerful ability of our model to conditionally generate point clouds across multiple modalities, including text, images, and point clouds. We also showcased the temporal continuity and inter-frame consistency of our model on the SemanticKITTI dataset. However, there is still room for further exploration in terms of temporal continuity, and we aim to unify the framework across more modalities. In particular, the results of generating point clouds from images could be improved. This will be a direction for our continued exploration moving forward.
